Polyregular functions on unordered trees of bounded height

We consider injective first-order interpretations that input and output trees of bounded height. The corresponding functions have polynomial output size, since a first-order interpretation can use a k-tuple of input nodes to represent a single output node. We prove that the equivalence problem for such functions is decidable, i.e. given two such interpretations, one can decide whether, for every input tree, the two output trees are isomorphic. We also give a calculus of typed functions and combinators which derives exactly injective first-order interpretations for unordered trees of bounded height. The calculus is based on a type system, where the type constructors are products, coproducts and a monad of multisets. Thanks to our results about tree-to-tree interpretations, the equivalence problem is decidable for this calculus. As an application, we show that the equivalence problem is decidable for first-order interpretations between classes of graphs that have bounded tree-depth. In all cases studied in this paper, first-order logic and MSO have the same expressive power, and hence all results apply also to MSO interpretations.

==> lower-bound.tex <==
\subsection{A non-elementary lower bound} 
The quantifier-elimination procedure in Lemma~\ref{lem:quantifier-elimination} incurs a non-elementary blow-up. 
We finish this section by showing that this blowup is indeed necessary. This is a standard lower bound for \fo logic, and it follows the same lines as similar lower bounds for satisfiability of \fo or \mso logics over strings or trees.
 
\begin{lemma}\label{lem:lower-bound}
 The following problem has non-elementary complexity: given a first-order sentence $\varphi$ over the vocabulary of some multiset type $\Sigma$, decide if the sentence is true in some element of $\Sigma$. 
\end{lemma}
\begin{proof}The proof follows~\cite[Section 10.3]{flumGrohe}.
 By induction on $k \in \set{0,1,\ldots}$, we define a \emph{$k$-tree} to be any element of $\multisets^k 1$ that can be obtained as follows. For $k=0$ there is only one $0$-tree, namely the unique element of $\multisets^0 1 = 1$. A $(k+1)$-tree is defined to be any multiset that contains only $k$-trees, and which does not contain any $k$-tree more than once; in other words it is a set of $k$-trees viewed as a multiset. If we define $f(k)$ to be the number of $k$-trees, then 
\begin{align*}
f(k+1) =
2^{f(k)}
\end{align*}
and therefore the number of $k$-trees is the non-elementary in $k$. We use the following linear ordering on $k$-trees: we view a $(k+1)$-tree as a bit vector indexed by $k$-trees, and order such bit vectors lexicographically, using the inductively defined order on $k$-trees. By a simple induction on $k$, one proves the following claim (see~\cite[Lemma 10.21]{flumGrohe}). 
\begin{claim}
 For every $k \le \ell$ there is a first-order formula $\varphi(x,y)$ over the vocabulary of $\multisets^\ell 1$ such that 
 \begin{align*}
 A,a,b \models \varphi
 \end{align*}
 holds if and only if $a$ and $b$ represents sub-trees of $A$ that are both $k$-trees, and such that $a$ is smaller or equal to $b$ in the order on $k$-trees. Furthermore, the size of this formula is polynomial in $k$ if we use circuit representation, i.e.~ if the size of a formula is the number of distinct sub-formulas.
\end{claim}

As already mentioned, a $(k+1)$-tree can be seen as bit vector of length $f(k)$. By using such bit vectors to represent configurations of Turing machines with space $f(k)$, we can use the above claim to get a reduction to the problem in Lemma~\ref{lem:lower-bound} from the following problem:
\begin{itemize}
\item {\bf Input.} A Turing machine $M$ and $k \in \set{0,1,\ldots}$;
\item {\bf Output.} Does $M$ have an accepting run that uses space at most $f(k)$? 
\end{itemize}
The reduction is either polynomial time or exponential time, depending on whether we use tree or circuit representation for formulas. In either case, the reduction proves Lemma~\ref{lem:lower-bound}, since the above problem cannot be decided in elementary time.
\end{proof}
